Multi-Temporal Land Cover Classification with Sequential Recurrent Encoders

Earth observation (EO) sensors deliver data with daily or weekly temporal resolution. Most land use and land cover (LULC) approaches, however, expect cloud-free and mono-temporal observations. The increasing temporal capabilities of today's sensors enables the use of temporal, along with spectral and spatial features. Domains, such as speech recognition or neural machine translation, work with inherently temporal data and, today, achieve impressive results using sequential encoder-decoder structures. Inspired by these sequence-to-sequence models, we adapt an encoder structure with convolutional recurrent layers in order to approximate a phenological model for vegetation classes based on a temporal sequence of Sentinel 2 (S2) images. In our experiments, we visualize internal activations over a sequence of cloudy and non-cloudy images and find several recurrent cells, which reduce the input activity for cloudy observations. Hence, we assume that our network has learned cloud-filtering schemes solely from input data, which could alleviate the need for tedious cloud-filtering as a preprocessing step for many EO approaches. Moreover, using unfiltered temporal series of top-of-atmosphere (TOA) reflectance data, we achieved in our experiments state-of-the-art classification accuracies on a large number of crop classes with minimal preprocessing compared to other classification approaches.

==> tables/approaches.tex <==
\def\cellwidth{1cm}

% short alias for multocol
\newcommand{\twocells}[1]{\multicolumn{2}{c|}{#1}}
\newcommand{\Vtwocells}[1]{\multicolumn{2}{|>{\hsize=\dimexpr2\hsize+2\tabcolsep+\arrayrulewidth\relax}X|}{#1}}
%{\Large %  
\begin{tabularx}{\textwidth}{c|cc|cc|cc|cc|cc|cc|cc|cc|cc}
	%{R{1cm}|R{\cellwidth}|L{\cellwidth}|R{\cellwidth}|L{\cellwidth}|R{\cellwidth}|L{\cellwidth}|R{\cellwidth}|L{\cellwidth}|R{\cellwidth}|L{\cellwidth}|R{\cellwidth}|L{\cellwidth}|R{\cellwidth}|L{\cellwidth}}
 & 
 \twocells{this approach} & 
 \twocells{\citet{Russwurm17:TVM}} & 
 \twocells{\citet{Foerster2012}} & 
 \twocells{\citet{Hao15}} & 
 \twocells{\citet{conrad2010}} & 
 \twocells{\citet{conrad2014}} & 
 \twocells{\citet{Jakubauskas2002}} & 
 \twocells{\citet{Barragan2011}} &
 \twocells{\citet{Siachalou2015}} \\ \hline
 
%notes & 
%\Vtwocells{ConvRNN, Bavaria, Sentinel 2, no pre/postprocessing} & 
%\Vtwocells{RNN, Bavaria, Sentinel 2, multitemporal, minor pre/postprocessing} & 
%\Vtwocells{multiyear NDVI timeseries, Landsat 7, North Germany, additional phenological metrics} & 
%\Vtwocells{Kansas, Modis Random Forests} & 
%\Vtwocells{high resolution, SPOT ASTER, arid central asia, object based} & 
%\Vtwocells{high resolution, SPOT ASTER, arid central asia, object based} &
%\Vtwocells{harmonic analysis, harmonic analysis NDVI} & 
%\Vtwocells{Object based image analysis} &
%\Vtwocells{} 
%\\ \hline

% low: drownload -> crop -> classify
% medium: download -> atmopheric correction/freature extraction/ model design -> classify
% high: same as medium with additionally required information (e.g. phenological correction)
datacost/access & 
\Vtwocells{low} & % us
\Vtwocells{low} &  % us17
\Vtwocells{medium} & % Foe
\Vtwocells{low} & % Ha
\Vtwocells{high} &  % Conrad10 two satellites spot https://en.wikipedia.org/wiki/SPOT_(satellite)aster $$ and Aster https://en.wikipedia.org/wiki/Advanced_Spaceborne_Thermal_Emission_and_Reflection_Radiometer
\Vtwocells{high} &  % Conrad14 RapidEye and SPOT
\Vtwocells{medium} & %Jaku % https://en.wikipedia.org/wiki/Advanced_very-high-resolution_radiometer, daily repeat 1km GSD
\Vtwocells{medium} & % PeBarr
\Vtwocells{medium} % Sia Landsat free/ Rapideye eypensive
\\ \hline

% possible operations
% download, crop, atmospheric correction, feature extraction, model design, postprocessing, voting, classification steps

% low: drownload -> crop -> classify
% medium: download -> atmopheric correction/freature extraction/ model design -> classify
% high: same as medium with additional required information (e.g. agro-meteorological information) or additional coregistration
pre/postprocessing &
\Vtwocells{low} & %us % 2
\Vtwocells{medium} & %us17 % cloud mask required for training/ classification at each time -> voting at postprocessing 
\Vtwocells{high} & %Foe  % requires NDVI statistics and additional phenological information
\Vtwocells{medium} & %conrad10
\Vtwocells{high} & %conrad14 % + atmospheric correction/ coregistration
\Vtwocells{medium} & %Jaku
\Vtwocells{medium} & %PeBarr
\Vtwocells{medium} %Sia 
\\ \hline

features &
\Vtwocells{TOA reflectance} & %us
\Vtwocells{BOA reflectance} & %us17
\Vtwocells{phen. normalized NDVI statistics} & %Foe
\Vtwocells{NDVI statustics} & %Hao
\Vtwocells{VIs} & %Conrad10
\Vtwocells{VIs} & 
\Vtwocells{NDVI harmonics} & 
\Vtwocells{VIs} &
\Vtwocells{TOA reflectance} 
\\ \hline

classification &
\Vtwocells{ConvRNN} & 
\Vtwocells{RNN} & 
\Vtwocells{Decision Tree} & 
\Vtwocells{Random Forrest} & %Hao
\Vtwocells{OBIA\footnote{Object based image analysis} and Decision Tree} & 
\Vtwocells{OBIA and Random Forrest} & 
\Vtwocells{discriminant analysis} & 
\Vtwocells{OBIA\footnote{Object based image analysis} and Decision Tree} & 
\Vtwocells{OBIA\footnote{Object based image analysis} and HMMs} 
\\ \hline

sensor &
\Vtwocells{\satellite{Sentinel 2}} & 
\Vtwocells{\satellite{Sentinel 2}} & 
\Vtwocells{\satellite{Landsat 4/5/7}} & 
\Vtwocells{\satellite{MODIS}} & 
\Vtwocells{\satellite{SPOT},\satellite{Aster}} & 
\Vtwocells{\satellite{SPOT}, \satellite{RapidEye} and \satellite{Quickbird}} & 
\Vtwocells{\satellite{AVHRR}} & 
\Vtwocells{\satellite{Aster}} & 
\Vtwocells{\satellite{Landsat 7}, \satellite{RapidEye}} \\ \hline

region &
\Vtwocells{south Germany} & %us
\Vtwocells{south Germany} & %us17
\Vtwocells{north Germany} & %Foe
\Vtwocells{Kansas, USA} & %Hao
\Vtwocells{Uzbekistan} & %con10
\Vtwocells{Uzbekistan} & %con14
\Vtwocells{Kansas, USA} & %Jaku
\Vtwocells{California, USA} & %PeBarr
\Vtwocells{Greece} %Siach 
\\ \hline

support [ha]          & 
\twocells{76665 ha} & %us
\twocells{48852 ha}  & %us17
\twocells{1619 ha} & %foe
\twocells{148900 ha} & %Ha
\twocells{} & %Con10
\twocells{} & %Con14
\twocells{} & % Jaku
\twocells{7500 ha \footnote{combined train and test}} %Sia
\\ %\hline

support [px]          & 
\twocells{$7666505 px^{10m}$} & %us
\twocells{$542785 patches$ }  & %us17
\twocells{$17993 px^{30m}$ \footnote{estimated from Landsat pixelsize and area} } & %Foe
\twocells{$5956 px^{500m}$} & %Hao
\twocells{$196 parcels$} & %Conrad10
\twocells{$511 parcels$} & %Conrad14
\twocells{} & % Jaku 
\twocells{} & % PeBarr 
\twocells{$3264 parcels$} % Sia 
\\ \hline

overall accuracy &
\twocells{} & % us 
\twocells{74.3} & %us17
\twocells{72.8} & %Foe
\twocells{88.81} & %Hao
\twocells{80.0} & %Conrad10
\twocells{85.7} & %Conrad14
\twocells{51.70} & % calculated from provided confusion matrix oa=(471+33+120+57+241+687)/3112
\twocells{79} &
\twocells{92.5} 
\\ \hline

kappa &
\twocells{} & 
\twocells{67.4} & 
\twocells{} & 
\twocells{} & 
\twocells{} & 
\twocells{} & 
\twocells{75} &
\twocells{88.1} 
\\ \hline

classes &
\twocells{18} & %us
\twocells{18} & %us17
\twocells{11} & %Foe
\twocells{6} & %Ha
\twocells{6} & %con10
\twocells{17} & %con14
\twocells{6} & % Jaku
\twocells{13} & %PeBarr
\twocells{6} % sia
\\ \hline

%                 ours     RK17    Foerster     Hao        Conrad10      Jakubausk       P. Barragan
%crop             &PA &UA &PA &UA &PA   &UA & PA   & UA   & PA  & UA  & & & PA & UA & PA & UA \\% \cline{2-15}
%\hline                                                               
%corn             &95 &87 &70 &77 &64.6 &15 &87    &84    &     &     & & &44  &32  &83  &83  \\% \cline{2-15}
%wheat            &90 &89 &62 &88 &92   &41 &100   &97    &     &     & & &    &    &77  &79  \\% \cline{2-15}
%wheat/soybeans   &   &   &   &   &     &   &81    &91    &90.9 &71.4 & & &41  &66  &    &    \\% \cline{2-15}
%wheat/rice 	     &   &   &   &   &     &   &      &      &89.7 &83.9 & & &    &    &    &    \\% \cline{2-15}
%winter barley    &88 &87 &58 &91 &     &   &      &      &     &     & & &    &    &    &    \\% \cline{2-15}
%meadow           &77 &68 &60 &75 &     &91 &      &      &     &     & & &72  &67  &85  &69  \\% \cline{2-15}
%potato           &76 &86 &57 &57 &0    &0  &      &      &     &     & & &    &    &    &    \\% \cline{2-15}
%rape             &90 &93 &74 &86 &93   &49 &      &      &     &     & & &    &    &    &    \\% \cline{2-15}
%summer barley    &76 &84 &63 &74 &     &   &      &      &     &     & & &    &    &    &    \\% \cline{2-15}
%sugar beet       &68 &96 &69 &52 &100  &0  &      &      &     &     & & &    &    &    &    \\% \cline{2-15}
%winter triticale &45 &62 &41 &30 &     &   &      &      &     &     & & &    &    &    &    \\% \cline{2-15}
%hop              &76 &82 &68 &75 &     &   &      &      &     &     & & &    &    &    &    \\% \cline{2-15}
%oats             &50 &67 &48 &37 &     &   &      &      &     &     & & &    &    &75  &70  \\% \cline{2-15}
%rye              &58 &52 &59 &34 &71   &57 &      &      &     &     & & &    &    &50  &100 \\% \cline{2-15}
%winter spelt     &51 &61 &65 &17 &     &   &      &      &     &     & & &    &    &    &    \\% \cline{2-15}
%beans            &62 &87 &66 &45 &     &   &      &      &     &     & & &    &    &    &    \\% \cline{2-15}
%soybeans         &40 &85 &65 &27 &     &   &83    &80    &     &     & & &    &    &    &    \\% \cline{2-15}
%asparagus        &70 &81 &68 &33 &     &   &      &      &     &     & & &    &    &    &    \\% \cline{2-15}
%vegetable        &0  &0  &   &   &     &   &      &      &     &     & & &    &    &    &    \\% \cline{2-15}
%peas             &73 &74 &55 &40 &     &   &      &      &     &     & & &    &    &    &    \\% \cline{2-15}
%alfalfa          &   &   &   &   &     &   &86    &93    &     &     & & &48  &40  &80  &72  \\% \cline{2-15}
%almond           &   &   &   &   &     &   &      &      &     &     & & &    &    &60  &83  \\% \cline{2-15}
%barley           &   &   &   &   &77   &82 &      &      &     &     & & &    &    &    &    \\% \cline{2-15}
%cotton           &   &   &   &   &     &   &      &      &83.8 &81.6 & & &    &    &    &    \\% \cline{2-15}
%fallow           &   &   &27 &9  &77   &51 &      &      &85.7 &100  & & &50  &37  &    &    \\% \cline{2-15}
%milo             &   &   &   &   &     &   &      &      &     &     & & &27  &16  &    &    \\% \cline{2-15}
%oilseed crops    &   &   &   &   &92   &75 &      &      &     &     & & &    &    &    &    \\% \cline{2-15}
%other            &   &   &   &   &     &   &      &      &55.2 &53.3 & & &    &    &    &    \\% \cline{2-15}
%rice             &   &   &   &   &     &   &      &      &75.0 &96.8 & & &    &    &95  &93  \\% \cline{2-15}
%safflower        &   &   &   &   &     &   &      &      &     &     & & &    &    &73  &71  \\% \cline{2-15}
%sorghum          &   &   &   &   &     &   &84    &88    &     &     & & &    &    &    &    \\% \cline{2-15}
%summer grain     &   &   &   &   &72.2 &0  &      &      &     &     & & &    &    &    &    \\% \cline{2-15}
%sunflower        &   &   &   &   &     &   &      &      &     &     & & &    &    &85  &89  \\% \cline{2-15}
%tomato           &   &   &   &   &     &   &      &      &     &     & & &    &    &79  &82  \\% \cline{2-15}
%vineyard         &   &   &   &   &     &   &      &      &     &     & & &    &    &90  &75  \\% \cline{2-15}
%walnut           &   &   &   &   &     &   &      &      &     &     & & &    &    &73  &75  \\% \cline{2-15}

\end{tabularx}                  


==> tables/gru256.tex <==
\cn{sugar beet}	&	95	&	78	&	85	&	59k	&	89	&	79	&	83	&	94k	\\
\cn{summer oat}	&	86	&	68	&	76	&	36k	&	64	&	63	&	63	&	38k	\\
\cn{meadow}		&	91	&	86	&	88	&	233k	&	88	&	85	&	87	&	242k	\\
\cn{rape}		&	95	&	90	&	93	&	125k	&\best{96}	&	96	&\best{96}	&	114k	\\
\cn{hop}		&\best{96}	&	87	&	92	&	51k	&	93	&	75	&	83	&	53k	\\
\cn{winter spelt}	&\worst{55}	&	81	&	66	&	38k	&	75	&	47	&	58	&	31k	\\
\cn{winter triticale}&	69	&	56	&	62	&	65k	&	62	&	57	&	60	&	64k	\\
\cn{beans}		&	92	&	87	&	90	&	27k	&	93	&	63	&	75	&	28k	\\
\cn{peas}		&	93	&	71	&	80	&	9k	&\worst{61}	&\worst{41}	&\worst{49}	& 	6k	\\
\cn{potato}		&	91	&	88	&	90	&	125k	&	95	&	74	&	83	&	140k	\\
\cn{soybeans}	&	98	&	80	&	88	&	21k	&	76	&	80	&	78	&	26k	\\
\cn{asparagus}	&	89	&	79	&	84	&	20k	&	82	&	77	&	79	&	19k	\\
\cn{winter wheat}	&	88	&	93	&	90	&	806k	&	90	&	95	&	92	&	783k	\\
\cn{winter barley}	&	95	&	87	&	91	&	258k	&	93	&	92	&	92	&	255k	\\
\cn{winter rye}	&	86	&\worst{47}	&\worst{61}	&	43k	&	77	&	62	&	69	&	30k	\\
\cn{summer barley}	&	88	&	83	&	85	&	73k	&	78	&	88	&	83	&	91k	\\
\cn{maize}		&	92	&\best{96}	&\best{94}	&	920k	&	92	&\best{97}	&	94	&	876k	\\
\addlinespace
\textbf{weight. avg}	&\textbf{90}	&\textbf{90}	&\textbf{90}	&		&\textbf{89}	&\textbf{90}	&\textbf{89}	&		\\

